Clustering and Labelling Auction Fraud Data

Although shill bidding is a common auction fraud, it is however very tough to detect. Due to the unavailability and lack of training data, in this study, we build a high-quality labeled shill bidding dataset based on recently collected auctions from eBay. Labeling shill biding instances with multidimensional features is a critical phase for the fraud classification task. For this purpose, we introduce a new approach to systematically label the fraud data with the help of the hierarchical clustering CURE that returns remarkable results as illustrated in the experiments.

==> Last Version/RelatedWorkConf2August18.tex <==
\section{Related Work} 
Many researchers utilized data clustering to examine auctions from different angles, such as studying the dynamics of auction prices and bidder behaviour. For instance, \cite{jank2009studying} introduced an approach to model and analyze the price formation as well as its dynamics to characterize the heterogeneity of the price formation process. The proposed functional objects represent the price process by accommodating the structure format of bidding data on eBay. Then, the curve clustering is used to partition auctions by grouping similar price profiles. Finally, differential equations are used to specify the price of each group.  

\cite{ford2010identifying} measured the similarity of bidder behaviour with specific attributes, such as bidder feedback rating, average increment difference and number of bids. Then, a centroid-based hierarchical clustering approach is presented to group similar bidders. Each produced cluster is then labeled manually according to the overall bidder behaviour in that cluster. 

 \cite{lei2012k} suggested a SB detection model based on k-mean clustering. The latter groups similar winners in one class to differentiate between actual buyers and shill bidders. There are four features that represent a buyer: ``the absolute average discrepancy of buyer bids", ``how long the buyer has been in the auction", ``the times of buyer bids" and "the average response time of the buyer". Based on these features, k-mean classifies bidders into only two clusters: general buyers and shill bidders. However, we believe the second and third features do not really reflect SB since a buyer might be very interested in winning the auction. Besides, there are stronger patterns that highly identify SB.  Since SB behaviour is somehow similar to real bidding \cite{Dong2009}, there is a possibility that some SB samples fall in the normal class.

\cite{cui2013bidding} proposed a two-step clustering model to recognize bidding strategies. The hierarchical clustering is the first step to produce a dendrogram and an agglomeration schedule table to determine the optimal number of clusters.  The next step employs  k-mean clustering  {\bf to provide more details about the clusters: produce the content of clusters???}. The experiment operated on online auctions to validate the suggested model.  According to the agglomeration coefficients, the optimal number of clusters is three:  ``early bidding strategy", ``snipe bidding strategy", and the third one groups bidders that enter the auction early and remain for a long time. {\bf The label of these clusters is given w. r. t. the values of four features.  There is no particular automatic mechanism suggested for labeling the samples. these two sentences are in contradictions???} 

\cite{zhang2013feedback} proposed a model based on hedonic regression and fuzzy logic expert system (FLES) to analyze bidder behaviour. The hedonic regression is used to select key variables passed to FLES to produce a knowledge base about the relationships between variables, like auction characteristics.  Since the examined data have no relational information, k-mean is employed to obtain the minimum squared-error clusters. So, each training sample is classified to low, medium or high membership degree. The issue here is that the study is based on an outdated dataset (2004). Also, there is a potential for fabricating feedback ratings conducted between shill bidders and fraudulent bidder rings \cite{ford2010identifying}. 

More recently, \cite{gupta2015online} applied k-mean clustering to categorize bidder habits. The observations are obtained from the {\bf clustering technique- which one} and then passed to the Baum-Welch algorithm and Hidden Markov Model. Three main clusters were suggested: {\bf low, medium and high what is the meaning???}. The experiment showed that only two simple features were given to the clustering technique to determine the model parameters. If the number of features is increased, then different parameters are produced. {\bf This may influence the detection model results}. Also, the clustering is based on a dataset that is not adequately described, and only ten samples were considered for explaining the results. 

Lastly, \cite{ganguly2018online} applied hierarchical clustering to group users with similar bidding behaviour.  The centroid linkage is used as the similarity measure. The described SB patterns were measured for all the bidders of each cluster.  The authors introduced a semi-automatic technique to label each cluster according to its characteristics and the general users' behaviour in that cluster.

==> RelatedWorkConf2August18.tex <==
\section{Related Work} 
Many researchers utilized data clustering to examine auctions from different angles, such as studying the dynamics of auction prices and bidder behaviour. For instance, \cite{jank2009studying} introduced an approach to model and analyze the price formation as well as its dynamics to characterize the heterogeneity of the price formation process. The proposed functional objects represent the price process by accommodating the structure format of bidding data on eBay. Then, the curve clustering is used to partition auctions by grouping similar price profiles. Finally, differential equations are used to specify the price of each group.  

\cite{ford2010identifying} measured the similarity of bidder behaviour with specific attributes, such as bidder feedback rating, average increment difference and number of bids. Then, a centroid-based hierarchical clustering approach is presented to group similar bidders. Each produced cluster is then labeled manually according to the overall bidder behaviour in that cluster. 

 \cite{lei2012k} suggested a SB detection model based on k-mean clustering. The latter groups similar winners in one class to differentiate between actual buyers and shill bidders. There are four features that represent a buyer: ``the absolute average discrepancy of buyer bids", ``how long the buyer has been in the auction", ``the times of buyer bids" and "the average response time of the buyer". Based on these features, k-mean classifies bidders into only two clusters: general buyers and shill bidders. However, we believe the second and third features do not really reflect SB since a buyer might be very interested in winning the auction. Besides, there are stronger patterns that highly identify SB.  Since SB behaviour is somehow similar to real bidding \cite{Dong2009}, there is a possibility that some SB samples fall in the normal class.

\cite{cui2013bidding} proposed a two-step clustering model to recognize bidding strategies. The hierarchical clustering is the first step to produce a dendrogram and an agglomeration schedule table to determine the optimal number of clusters.  The next step employs  k-mean clustering  {\bf to provide more details about the clusters: produce the content of clusters???}. The experiment operated on online auctions to validate the suggested model.  According to the agglomeration coefficients, the optimal number of clusters is three:  ``early bidding strategy", ``snipe bidding strategy", and the third one groups bidders that enter the auction early and remain for a long time. {\bf The label of these clusters is given w. r. t. the values of four features.  There is no particular automatic mechanism suggested for labeling the samples. these two sentences are in contradictions???} 

\cite{zhang2013feedback} proposed a model based on hedonic regression and fuzzy logic expert system (FLES) to analyze bidder behaviour. The hedonic regression is used to select key variables passed to FLES to produce a knowledge base about the relationships between variables, like auction characteristics.  Since the examined data have no relational information, k-mean is employed to obtain the minimum squared-error clusters. So, each training sample is classified to low, medium or high membership degree. The issue here is that the study is based on an outdated dataset (2004). Also, there is a potential for fabricating feedback ratings conducted between shill bidders and fraudulent bidder rings \cite{ford2010identifying}. 

More recently, \cite{gupta2015online} applied k-mean clustering to categorize bidder habits. The observations are obtained from the {\bf clustering technique- which one} and then passed to the Baum-Welch algorithm and Hidden Markov Model. Three main clusters were suggested: {\bf low, medium and high what is the meaning???}. The experiment showed that only two simple features were given to the clustering technique to determine the model parameters. If the number of features is increased, then different parameters are produced. {\bf This may influence the detection model results}. Also, the clustering is based on a dataset that is not adequately described, and only ten samples were considered for explaining the results. 

Lastly, \cite{ganguly2018online} applied hierarchical clustering to group users with similar bidding behaviour.  The centroid linkage is used as the similarity measure. The described SB patterns were measured for all the bidders of each cluster.  The authors introduced a semi-automatic technique to label each cluster according to its characteristics and the general users' behaviour in that cluster.
